Automated Black-Box Boundary Value Detection

The input domain of software systems can typically be divided into sub-domains for which the outputs are similar. To ensure high quality it is critical to test the software on the boundaries between these sub-domains. Consequently, boundary value analysis and testing has been part of the toolbox of software testers for long and is typically taught early to students. However, despite its many argued benefits, boundary value analysis for a given specification or piece of software is typically described in abstract terms which allow for variation in how testers apply it. Here we propose an automated, black-box boundary value detection method to support software testers in systematic boundary value analysis with consistent results. The method builds on a metric to quantify the level of boundariness of test inputs: the program derivative. By coupling it with search algorithms we find and rank pairs of inputs as good boundary candidates, i.e. inputs close together but with outputs far apart. We implement our AutoBVA approach and evaluate it on a curated dataset of example programs. Our results indicate that even with a simple and generic program derivative variant in combination with broad sampling over the input space, interesting boundary candidates can be identified.

==> abstract_long.tex <==
\begin{abstract}
The input domain of software systems can typically be divided into sub-domains for which the outputs are similar. To ensure high quality it is critical to test the software on the boundaries between these sub-domains. Not only can this help ensure that the behavior is correct on both sides of each boundary, it can also help ensure that the boundaries themselves are in the right place. Consequently, boundary value analysis and testing has been part of the toolbox of software testers for long and is typically taught early to students.
%in software engineering students in their education.

However, despite its many argued benefits there is less concrete advice on \textbf{how} to actually do boundary value analysis for a given specification or piece of software. The method is typically described and defined in abstract terms which allows for much variation in how testers actually apply it. This can hinder efficient results and makes them too dependent on the experience % background, 
and skills of the tester.

Here we propose an automated, black-box boundary value detection method to support software testers in systematic boundary value analysis with more consistent results. The method builds on a metric to quantify the level of boundariness of test inputs: the program derivative. By coupling it with search algorithms we can find and rank pairs of inputs that are good boundary candidates, i.e. inputs that are close together but whose outputs are far apart.

% Not clear how much we need to talk about the eval being "preliminary" etc given few sutes and simple input types but we can adjust this as we go along...
We implement our AutoBVA approach and evaluate it on a curated dataset of example programs. Our results indicate that even with a very simple and generic program derivative variant in combination with broad sampling over the input space, our approach can in short time identify interesting boundary candidates. The results indicate a potential benefit in combining and further investigating different local search methods in future research as the more sophisticated algorithm used in this study captured more interesting areas for two out of the four softwares under test. The method identifies potential faults and refinements for all of the investigated programs and we discuss their implications.
%four SUTS and discuss their implications.

%The purpose of this paper is to present a support mechanism for software testers that helps them reveal  potential faults in software.

%We detect areas of local change in software by means of automated input space exploration. Local change is measured using a blackbox approach and metrics relating inputs and outputs. We call neighboring inputs of relatively great local change boundary candidates.

%We also introduce a process to define boundary candidate reference lists for software, which serve as a benchmark to evaluate the exploration runs.
\end{abstract}
